Generalised Mermin-type non-locality arguments

We broadly generalise Mermin-type arguments on GHZ states, and we provide exact group-theoretic conditions for non-locality to be achieved. Our results are of interest in quantum foundations, where they yield a new hierarchy of quantum-realisable All-vs-Nothing arguments. They are also of interest to quantum protocols, where they find immediate application to a non-trivial extension of the hybrid quantum-classical secret sharing scheme of Hillery, Bu\v{z}ek and Berthiaume (HBB). Our proofs are carried out in the graphical language of string diagrams for dagger compact categories, and their validity extends beyond quantum theory to any theory featuring the relevant algebraic structures.

==> Generalised Mermin-type non-locality arguments/macros.tex <==
%%%% macros.tex by Stefano Gogioso
%%%% Version 26 Jul 2016 


%% Theorem environments - Comment out for certain journal submissions and for beamer 
	
	%% Counters and miscellaneous
	%	\newcounter{theorem_c} % Unified coutner for all theorem environments...
	% 	\numberwithin{theorem_c}{chapter} % ... numbered within chapters
	% 	\numberwithin{equation}{chapter} % Equations are also numbered within chapters (but have a separate counter)
	% 	\numberwithin{theorem_c}{section} % ... numbered within chapters
	%	\numberwithin{equation}{section} % Equations are also numbered within sections (but have a separate counter)
	% 	\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}} % Numbering of individual equations in align* environments. Usage: \numberthis \label{eqn_EquationTitle}

	%% Italic theorem environments
	% 	\theoremstyle{plain} 
	% 	\newtheorem{theorem}[theorem_c]{Theorem}
	% 	\newtheorem*{theorem*}{Theorem}
	% 	\newtheorem{kindatheorem}[theorem_c]{\textquotedblleft Theorem\textquotedblright}
	% 	\newtheorem{lemma}[theorem_c]{Lemma}
	% 	\newtheorem{corollary}[theorem_c]{Corollary}
		
	% 	\newtheoremstyle{exampstyle}
	% 	  {2mm} % Space above
	% 	  {2mm} % Space below
	% 	  {\itshape} % Body font
	% 	  {} % Indent amount
	% 	  {\bfseries} % Theorem head font
	% 	  {.} % Punctuation after theorem head
	% 	  {.5em} % Space after theorem head
	% 	  {} % Theorem head spec (can be left empty, meaning `normal')

	% %% Plain-text theorem environments
	% 	%\theoremstyle{definition}
	% 	\theoremstyle{exampstyle}
	% 	\newtheorem{definition}[theorem_c]{Definition}
	% 	\newtheorem{example}[theorem_c]{Example}
	% 	\newtheorem{remark}[theorem_c]{Remark}



%% General 
	\newcommand{\emptyArg}{\,\underline{\hspace{6px}}\,} % Underscore for omitted, anonymous arguments
	\newcommand{\inlineQuote}[1]{\textquotedblleft #1\textquotedblright} % Left-right quotes surrounding #1
	\newcommand{\TODO}{\textbf{[TODO]}} % A bold TODO placeholder
	\newcommand{\citeTODO}[1]{\textbf{[#1]}} % A bold citation placeholder
	\newcommand{\goodchi}{\protect\raisebox{2pt}{$\chi$}} % A chi letter raised at line level, for those instances where alignment is an issue
	\newcommand{\goodrho}{\protect\raisebox{2pt}{$\rho$}} % A rho letter raised at line level, for those instances where alignment is an issue
	\newcommand{\goodvdots}{\protect\raisebox{7pt}{\vdots}} % A \vdots simbol raised, for use in tikz nodes where vertical alignment is a problem 
	\newcommand{\verteq}{\rotatebox{90}{$\,=$}}


%% Sets, groups and algebra
	\newcommand{\Powerset}[1]{\mathcal{P}(#1)} % Powerset of #1
	\newcommand{\naturals}{\mathbb{N}} % Set of natural numbers
	\newcommand{\integers}{\mathbb{Z}} % Set of interer numbers
	\newcommand{\rationals}{\mathbb{Q}} % Set of rational numbers
	\newcommand{\reals}{\mathbb{R}} % Set of real numbers
	\newcommand{\complexs}{\mathbb{C}} % Set of complex numbers
	\newcommand{\integersMod}[1]{\mathbb{Z}_{#1}} % Set/group/ring of integers mod #1
	\newcommand{\modclass}[2]{#1 \; (\text{mod } #2)} % Equivalence class of integers mod #2 corresponding to representative #1
	\newcommand{\restrict}[2]{\left. #1 \right\vert_{#2}} % Restriction of function/morphism #1 to subset/subobject #2
	\newcommand{\domain}[1]{\operatorname{dom}#1} % Domain of function/morphism #1
	\newcommand{\codomain}[1]{\operatorname{codom}#1} % Domain of function/morphism #1
	\newcommand{\support}[1]{\operatorname{supp}#1} % Domain of function/morphism #1
	\newcommand{\cosupport}[1]{\operatorname{cosupp}#1} % Domain of function/morphism #1
	\newcommand{\inject}{\hookrightarrow} % Set-theoretic injection
	\newcommand{\Irreps}[1]{\operatorname{Irr}[#1]} % Set of irreps for group #1
	\newcommand{\nonstd}[1]{^\star\!#1}
	\newcommand{\starNaturals}{\nonstd{\naturals}} % Set of non-standard naturals
	\newcommand{\starIntegers}{\nonstd{\integers}} % Set of non-standard integers
	\newcommand{\starRationals}{\nonstd{\rationals}} % Set of non-standard rationals
	\newcommand{\starComplexs}{\nonstd{\complexs}} % Set of non-standard complex numbers
	\newcommand{\starReals}{\nonstd{\reals}} % Set of non-standard realsnumbers
	\newcommand{\singletonSet}{\textbf{1}}
	\newcommand{\normalSubgroup}{\trianglelefteq}

%% Logic 
	\newcommand{\iffdef}{\stackrel{def}{\iff}} % If and only if (by definition)
	\newcommand{\iffdeftemp}{\stackrel{\Delta}{\iff}} % If and only if (by definition, but notation limited to section/context) 
	%\newcommand{\eqdef}{\stackrel{def}{=}} % Equal (by definition)
	\newcommand{\eqdef}{:=} % Equal (by definition)	
	\newcommand{\eqdeftemp}{\stackrel{\Delta}{=}} % Equal (by definition, but notation limited to section/context) 
	\newcommand{\imply}{\Rightarrow} % Implies
	%\newcommand{\suchthat}[2]{\left\{#1 \: \text{ s.t. } \: #2\right\}} % Set of elements #1 such that condition #2 holds 
	\newcommand{\suchthat}[2]{\left\{#1 \: \middle\vert \: #2\right\}} % Set of elements #1 such that condition #2 holds 
	\newcommand{\turnstyle}{\models} % Entails


%% Topology, geometry and linear algebra 

	%% Inner products and traces
		\newcommand{\ket}[1]{\vert #1 \rangle} % Ket labelled #1
		\newcommand{\bra}[1]{\langle #1 \vert} % Bra labelled #1
		\newcommand{\braket}[2]{\langle #1 \vert #2 \rangle} % Inner product of bra labelled #1 with ket labelled #2
		\newcommand{\innerprod}[2]{\left( #1 , #2 \right)}
		\newcommand{\Dim}[1]{\operatorname{dim}#1} % Dimension of a space
		\newcommand{\Trace}[1]{\operatorname{Tr}[#1]} % Trace of an operator
		%\newcommand{\pTrace}[4]{\operatorname{Tr}_{#2,#3}^{#4}[#1]} % Trace of an operator
		\newcommand{\pTrace}[2]{\operatorname{Tr}_{#1}[#2]} % Trace of an operator
		\newcommand{\Norm}[2]{|| #2 ||_{#1}} % #1-norm of #2
		\newcommand{\decohSym}{\operatorname{dec}} % Decoherence map symbol
		\newcommand{\decoh}[1]{\decohSym_{#1}} % Decoherence map (for a given observable)
		\newcommand{\CPMdoubled}[1]{\textbf{double}\left[#1\right]}

	%% Kernels and images
		%\newcommand{\ker}[1]{\operatorname{ker}#1} % Kernel of a function
		\newcommand{\im}[1]{\operatorname{im}#1} % Image of a function
		\newcommand{\LinExt}[1]{\operatorname{LinExt}[#1]} % Linear extension of a function
		\newcommand{\RLinExt}[2]{#2\operatorname{-LinExt}[#1]} % R-linear extension of a function
		\newcommand{\Annihil}[1]{\operatorname{Ann}[#1]} % Annihilator subgroup of $G^\wedge$ for some subgroup $H \leq G$

	%% Sets and spans
		\newcommand{\neighborhoods}[1]{\mathfrak{N}_#1} % Set of neighborhoods of point #1
		\newcommand{\tangspace}[2]{T_{#1} \, #2} % Tangent space of point #2 in manifold #1
		\newcommand{\LinearEndoms}[1]{\operatorname{L}\left[#1\right]} % Set of linear endomorphisms of space #1
		\newcommand{\Span}[1]{\operatorname{Span}[#1]} % Span of element #1
		\newcommand{\Bounded}[1]{\operatorname{B}\left[#1\right]} % Space of bounded operators over #1
		\newcommand{\BoundedMaps}[2]{\operatorname{B}\big(#1,#2\big)} % Space of bounded operators over #1
		\newcommand{\LtwoSym}{\operatorname{L}^2} % Symbol for L2 spaces
		\newcommand{\Ltwo}[1]{\LtwoSym[#1]} % L2 space over space #1
		\newcommand{\ltwoSym}{\ell^2} % Symbol for l2 spaces
		\newcommand{\ltwo}[1]{\ltwoSym[#1]} % l2 space over space #1

	%% General purpose space names 
		\newcommand{\SpaceH}{\mathcal{H}} 
		\newcommand{\SpaceG}{\mathcal{G}}
		\newcommand{\SpaceK}{\mathcal{K}}
		\newcommand{\SpaceA}{\mathcal{A}}
		\newcommand{\SpaceB}{\mathcal{B}}
		\newcommand{\GroupG}{\mathbb{G}}
		\newcommand{\GroupH}{\mathbb{H}}
		\newcommand{\GroupK}{\mathbb{K}}


%% Category Theory 

	%% Morphisms 
		\newcommand{\isom}{\cong} % Isomorphism
		\newcommand{\iso}{\cong} % Another definition for isomorphism
		\newcommand{\epim}{\twoheadrightarrow} % Epimorphism
		\newcommand{\monom}{\rightarrowtail} % Monomorphism
		\newcommand{\id}[1]{id_{#1}} % Identity morphism of object #1
		\newcommand{\pushforward}[1]{#1_\star} % Pushforward associated with morphism #1
		\newcommand{\pullback}[1]{#1^\star} % Pullback associated with morphism #1

	%% Monoidal categories
		\newcommand{\tensor}{\otimes} % Monoidal tensor
		\newcommand{\tensorUnit}{I} % Monoidal tensor unit
		\newcommand{\cartesianTensor}{\times} % Cartesian product

	%% Homsets 
		\newcommand{\Hom}[3]{\operatorname{Hom}_{\,#1}\left[#2,#3\right]} % Set of morphisms in category #1 from object #2 to object #3
		\newcommand{\Nat}[3]{\operatorname{Nat}_{#1}[#2,#3]} % Set of natural transformations in functor category #1 from functor #2 to functor #3
		\newcommand{\Endoms}[2]{\operatorname{End}_{\,#1}\left[#2\right]} % Set of endomorphisms in category #1 for object #2
		\newcommand{\Automs}[2]{\operatorname{Aut}_{\,#1}\left[#2\right]} % Set of autoomorphisms in category #1 for object #2
		\newcommand{\Subobjs}[2]{\operatorname{Sub}_{#1}[#2]} % Set of subobjects (usually mono) in category #1 for object #2
		\newcommand{\Subsys}[2]{\operatorname{Subsys}_{#1}[#2]} % Set of subsystems (not necessarily mono) in category #1 for object #2
		\newcommand{\States}[2]{\operatorname{States}_{#1}[#2]} % Set of states in (monoidal) category #1 for object #2 

	%% Canonical categories
		\newcommand{\DiffCategory}{\operatorname{Diff}} % Category of differentiable manifolds
		\newcommand{\TopCategory}{\operatorname{Top}} % Category of topological spaces
		\newcommand{\SetCategory}{\operatorname{Set}} % Category of sets
		\newcommand{\CatCategory}{\operatorname{Cat}} % Category of small categories
		\newcommand{\SitesCategory}{\operatorname{Sites}} % Category of small sites

		\newcommand{\GrpCategory}{\operatorname{Grp}} % Category of groups
		\newcommand{\fGrpCategory}{\operatorname{fGrp}} % Category of finite groups
		\newcommand{\AbCategory}{\operatorname{Ab}} % Category of abelian groups
		\newcommand{\fAbCategory}{\operatorname{fAb}} % Category of finite abelian groups
		\newcommand{\fMonCategory}{\operatorname{fMon}} % Category of finite monoids
		\newcommand{\fComMonCategory}{\operatorname{fCommMon}} % Category of finite commutative monoids
		\newcommand{\CMonCategory}{\operatorname{CMon}} % Category of commutative monoids
		\newcommand{\RMatCategory}[1]{#1\operatorname{-Mat}} % Category of finite sets and matrices valued in a semiring R 
		%\newcommand{\fRfreeModCategory}[1]{#1\operatorname{-Mod}_{fd}^{free}}
		\newcommand{\fRfreeModCategory}[1]{\RMatCategory{#1}} % Category of finite-dimensional free R-modules (R field, ring, semiring...)
		\newcommand{\fRModCategory}[1]{#1\operatorname{-Mod}_{fd}} % Category of finite-dimensional R-modules (R field, ring, semiring...)
		\newcommand{\RModCategory}[1]{#1\operatorname{-Mod}} % Category of R-modules (R field, ring, semiring...)
		\newcommand{\fVectCategory}[1]{#1\operatorname{-Vect}_{fd}} % Category of finite-dim R-vector spaces (R field...)
		\newcommand{\VectCategory}[1]{#1\operatorname{-Vect}} % Category of R-vector spaces (R field...)

		\newcommand{\HilbCategory}{\operatorname{Hilb}} % Category of Hilbert spaces
		\newcommand{\sHilbCategory}{\operatorname{sHilb}} % Category of Hilbert spaces
		\newcommand{\fdHilbCategory}{\operatorname{fdHilb}} % Category of finite-dimensional Hilbert spaces
		\newcommand{\fdSubIsomsCategory}{\operatorname{fdSubIsoms}} % Category of finite-dimensional Hilbert spaces
		\newcommand{\fdCPSUCategory}{\operatorname{fdCPSU}} % Category of finite-dimensional Hilbert Spaces and Completely Positive Sub-Unital maps
		\newcommand{\RelCategory}{\operatorname{Rel}} % Category of sets and relations
		\newcommand{\PInjCategory}{\operatorname{PInj}} % Category of sets and partial injections
		\newcommand{\fRelCategory}{\operatorname{fRel}} % Category of finite sets and relations
		\newcommand{\fRelPTEP}{\operatorname{fRel}} % Process theory with environments and purification of finite sets and relations
		\newcommand{\fPInjCategory}{\operatorname{fPInj}} % Category of finite sets and partial injections
		\newcommand{\fBijCategory}{\operatorname{fBij}} % Category of finite sets and bijections
		\newcommand{\fInjCategory}{\operatorname{fInj}} % Category of finite sets and injections
		\newcommand{\fPFunCategory}{\operatorname{fPFun}} % Category of finite sets and partial functions
		\newcommand{\fPFunPTEP}{\operatorname{fPFun}} % Process theory with environments and purification of finite sets and partial functions
		\newcommand{\fSetCategory}{\operatorname{fSet}} % Category of finite sets and total functions
		\newcommand{\fFunCategory}{\fSetCategory} % Category of finite sets and total functions
		\newcommand{\fFunPTEP}{\operatorname{fFun}} % Process theory with environments and purification of finite sets and total functions
		\newcommand{\fStochCategory}{\operatorname{fStoch}} % Category of finite sets and stochastic maps
		%\newcommand{\fStochCategory}[1]{\operatorname{fStoch}_{#1}} % Category of finite sets and stochastic maps over a semiring
		\newcommand{\starHilbCategory}{^\star\!\HilbCategory} % Category of omega-truncated non-standard hilbert spaces


	%% General-purpose category names
		\newcommand{\CategoryC}{\mathcal{C}}
		\newcommand{\CategoryD}{\mathcal{D}}
		\newcommand{\CategoryM}{M}

	%% Category operators and functors
		\newcommand{\obj}[1]{\operatorname{obj} \, #1} % Set of objects of category #1
		\newcommand{\OpCategory}[1]{#1^{\operatorname{op}}} % Op-category of category #1
		\newcommand{\CategoryObjs}[1]{\operatorname{obj} \, #1} % Another notatino for the set of objects of category #1
		\newcommand{\FullSubcat}[2]{\langle #2 \rangle_{#1}} % The full subcategory of #1 generated by #2
		\newcommand{\SliceCat}[2]{#1 / #2} % Slice category obtained from category #1 over objects #2
		\newcommand{\CosliceCat}[2]{#2 \backslash #1} % Co-slice category obtained from category #1 over objects #2
		\newcommand{\Symmetries}[1]{\Automs{#1}{\emptyArg}}  % Category of symmetries of objects of category #1
		\newcommand{\LocaleCategory}[1]{\mathcal{O}(#1)} % Locale category of topological space #1
		\newcommand{\CPMCategory}[1]{\operatorname{CPM}[#1]} % Selinger's CPM category
		\newcommand{\CPCategory}[1]{\operatorname{CP}[#1]} % Bob/Chris's conjugation-independent CP construction 
		\newcommand{\CPStarCategory}[1]{\operatorname{CP}^\ast[#1]} % Chris's CP star construction 
		\newcommand{\ClassicalCategory}[1]{\operatorname{K}[#1]} % Category with the same morphisms of #1, but objects pairs (object, classical structure) 
		\newcommand{\CausalSubCategory}[1]{#1_{\smallTraceSym}}
		\newcommand{\DoubledCategory}[1]{\operatorname{Double}\left[#1\right]}


%% CQM stuff
	\newcommand{\classicalStates}[1]{K(#1)} % Classical states for a $\dagger$-qSFA
	\newcommand{\phaseGroup}[1]{P(#1)} % Phase group for a $\dagger$-qSFA
	\newcommand{\phasegate}[1]{P_{#1}}
	\newcommand{\GHZstate}[1]{GHZ_{#1}}
	\newcommand{\CPstates}[1]{\mathcal{L}[#1]}



%% Monadic dynamics

	\newcommand{\monad}{T} % General-purpose monad symbol
	\newcommand{\unit}[1]{\eta_{#1}} % Monad unit over object #1
	\newcommand{\mult}[1]{\mu_{#1}} % Monad multiplication over object #1

	\newcommand{\timeobj}{\mathbb{T}} % Time object for the monad
	\newcommand{\timeaction}{\nu} % Time-translation action of the time object over itself (for the non-uniform case)
	\newcommand{\timeunit}{\unit{}} % Initial time (unit for the time object)
	\newcommand{\timemult}{\mult{}} % Time-translation (multiplication for the time object)
	\newcommand{\timediag}{\delta} % Diagonal for the time object
	\newcommand{\timeerase}{\epsilon} % Erasure for the time object 
	\newcommand{\timeinversion}[1]{i_{#1}} % Time-inversion operation over object #1
	\newcommand{\timeinverse}{\timeinversion{}} % Time-inversion (antipode)
	\newcommand{\foliate}[1]{\operatorname{foliate}_{#1}} % Foliation map AxTB -> T(AxB)
	\newcommand{\cofoliate}[1]{\operatorname{foliate'}_{#1}} % Foliation map TAxB -> T(AxB)

	\newcommand{\freehistory}[1]{\operatorname{freehist}_{#1}} % Free history of subsystem #1
	\newcommand{\FreeHistories}[2]{\operatorname{FreeHists}_{#1}[#2]} % Set of free histories in category #1 for object #2
	\newcommand{\concretehistory}[2]{\operatorname{hist}^{#1}_{#2}} % Concrete history of sybsystem #2 under dynamic #1
	\newcommand{\ConcreteHistories}[2]{\operatorname{Hists}_{#1}[#2]} % Set of concrete histories in category #1 for object #2
	\newcommand{\ConcreteHistoriesEMCategory}[1]{\prescript{H}{}{#1}} % Eilenberg-Moore category of concrete histories

	\newcommand{\timegenerator}{\partial_t} % Generator for the time object
	\newcommand{\futurespan}[1]{\span{#1}^+} % Future span for state #1
	\newcommand{\pastspan}[1]{\span{#1}^-} % Past span for state #1
	\newcommand{\causalfuture}[2]{\operatorname{J}^+_{#1}[#2]} % Causal future for state #1
	\newcommand{\causalpast}[2]{\operatorname{J}^-_{#1}[#2]} % Causal past for state #1
	\newcommand{\dynamicGenerator}[2]{\restrict{#1}{#2}} % Restriction of propagator #1 to time state #2


%% Coarse-graining and sheaf theory

	\newcommand{\comonad}{U} % General-purpose comonad symbol
	\newcommand{\counit}[1]{\epsilon_{#1}} % Comonad counit over object #1
	\newcommand{\comult}[1]{\nu_{#1}} % Comonad comultiplication over object #1
	\newcommand{\comonadFrak}{\mathfrak{U}} % frakture comonad symbol
	\newcommand{\sheafOfEventsSym}{\mathcal{E}} % Sheaf of events symbol
	\newcommand{\sheafOfEvents}[1]{\sheafOfEventsSym[#1]} % Sheaf of events symbol
	\newcommand{\restrictionMap}[2]{\operatorname{res}^{#1}_{#2}} % Restriction map for the sheaf of events
	\newcommand{\distributionFunctorSym}[1]{\mathcal{D}_{#1}} % Functor of R-distributions (symbol)
	\newcommand{\distributionFunctor}[2]{\distributionFunctorSym{#1}[#2]} % Functor of R-distributions
	\newcommand{\presheafOfDistributionsSym}[1]{\distributionFunctorSym{#1}\sheafOfEventsSym} % presheaf of distributions (symbol)
	\newcommand{\presheafOfDistributions}[2]{\presheafOfDistributionsSym{#1}[#2]} % presheaf of distributions (functor)
	\newcommand{\supportSubpresheafSym}{\mathbb{S}} % support subpresheaf (symbol)
	\newcommand{\supportSubpresheaf}[1]{\supportSubpresheafSym[#1]} % support subpresheaf (functor)
	

%% Inline Symbols for CQM 

	%% X structure / group structure
	\newcommand{\Xcolour}{Red}
	\newcommand{\XdotSym}{\hbox{\input{symbols/XdotSym.tex}}\!} % Dot
	\newcommand{\XmultSym}{\hbox{\input{symbols/timemultSym.tex}}\!} % Multiplication
	\newcommand{\XcomultSym}{\hbox{\input{symbols/timecomultSym.tex}}\!} % Comultiplication
	\newcommand{\XunitSym}{\hbox{\input{symbols/timeunitSym.tex}}\!} % Unit
	\newcommand{\XcounitSym}{\hbox{\input{symbols/timecounitSym.tex}}\!} % Counit
	\newcommand{\antipodeSym}{\hbox{\input{symbols/antipodeSym.tex}}\!} % Antipode (group inverse)
	\newcommand{\kpoints}[1]{K_{#1}} % Classical points of a given observable
	\newcommand{\Xkpoints}{\kpoints{\XdotSym}} % Classical points for the X observable
	
	%% Z structure / point structure
	\newcommand{\Zcolour}{YellowGreen}
	\newcommand{\ZdotSym}{\hbox{\input{symbols/ZdotSym.tex}}\!} % Dot
	\newcommand{\ZmultSym}{\hbox{\input{symbols/timematchSym.tex}}\!} % Multiplication
	\newcommand{\ZcomultSym}{\hbox{\input{symbols/timediagSym.tex}}\!} % Comultiplication
	\newcommand{\ZunitSym}{\hbox{\input{symbols/timematchunitSym.tex}}\!} % Unit
	\newcommand{\ZcounitSym}{\hbox{\input{symbols/trivialcharSym.tex}}\!} % Counit
	\newcommand{\Zkpoints}{\kpoints{\ZdotSym}} % Classical points for the Z observable

	%% alternative X structure / alternative group structure (e.g. for quotients)
	\newcommand{\Xaltcolour}{Purple}
	\newcommand{\XaltdotSym}{\hbox{\input{symbols/XaltdotSym.tex}}\!}
	\newcommand{\XaltmultSym}{\hbox{\input{symbols/internaltimemultSym.tex}}\!} % Multiplication
	\newcommand{\XaltcomultSym}{\hbox{\input{symbols/internaltimecomultSym.tex}}\!} % Comultiplication
	\newcommand{\XaltunitSym}{\hbox{\input{symbols/internaltimeunitSym.tex}}\!} % Unit
	\newcommand{\XaltcounitSym}{\hbox{\input{symbols/internaltimecounitSym.tex}}\!} % Counit
	\newcommand{\Xaltkpoints}{\kpoints{\XaltdotSym}} % Classical points for the alternative X observable
	
	%% alternative Z structure / alternative point structure
	\newcommand{\Zaltcolour}{Cyan}
	\newcommand{\ZaltdotSym}{\hbox{\input{symbols/ZaltdotSym.tex}}\!}
	\newcommand{\ZaltmultSym}{\hbox{\input{symbols/internaltimematchSym.tex}}\!} % Multiplication
	\newcommand{\ZaltcomultSym}{\hbox{\input{symbols/internaltimediagSym.tex}}\!} % Comultiplication
	\newcommand{\ZaltunitSym}{\hbox{\input{symbols/internaltimematchunitSym.tex}}\!} % Unit
	\newcommand{\ZaltcounitSym}{\hbox{\input{symbols/internaltrivialcharSym.tex}}\!} % Counit
	\newcommand{\Zaltkpoints}{\kpoints{\ZaltdotSym}} % Classical points for the alternative Z observable

	%% discrete structure (aliases the black structure)
	\newcommand{\Dcolour}{black!80}
	\newcommand{\DdotSym}{\hbox{\input{symbols/DdotSym.tex}}\!} % Dot	
	\newcommand{\DcomultSym}{\hbox{\input{symbols/DcomultSym.tex}}\!} % Comultiplication	
	\newcommand{\DmultSym}{\hbox{\input{symbols/DmultSym.tex}}\!} % Multiplication
	\newcommand{\DcounitSym}{\hbox{\input{symbols/DcounitSym.tex}}\!} % Counit
	\newcommand{\DunitSym}{\hbox{\input{symbols/DunitSym.tex}}\!} % Unit

	%% X structure in B/W (black structure)

	\newcommand{\Xbwcolour}{black!80}
	\newcommand{\XbwdotSym}{\hbox{\input{symbols/DdotSym.tex}}\!\!} % Dot	
	\newcommand{\XbwcomultSym}{\!\hbox{\input{symbols/DcomultSym.tex}}\!\!} % Comultiplication	
	\newcommand{\XbwmultSym}{\!\hbox{\input{symbols/DmultSym.tex}}\!\!} % Multiplication
	\newcommand{\XbwcounitSym}{\!\hbox{\input{symbols/DcounitSym.tex}}\!\!} % Counit
	\newcommand{\XbwunitSym}{\!\hbox{\input{symbols/DunitSym.tex}}\!\!} % Unit

	%% Z structure in B/W (white structure)
	\newcommand{\Zbwcolour}{white}
	\newcommand{\ZbwdotSym}{\hbox{\input{symbols/ZbwdotSym.tex}}\!\!} % Dot	
	\newcommand{\ZbwcomultSym}{\!\hbox{\input{symbols/ZbwcomultSym.tex}}\!\!} % Comultiplication	
	\newcommand{\ZbwmultSym}{\!\hbox{\input{symbols/ZbwmultSym.tex}}\!\!} % Multiplication	
	\newcommand{\ZbwcounitSym}{\!\hbox{\input{symbols/ZbwcounitSym.tex}}\!\!} % Counit
	\newcommand{\ZbwunitSym}{\!\hbox{\input{symbols/ZbwunitSym.tex}}\!\!} % Unit
	\newcommand{\ZbwleftDecohSym}{\hbox{\input{symbols/ZbwleftDecohSym.tex}}\!} % Left decoherence	
	\newcommand{\ZbwrightDecohSym}{\hbox{\input{symbols/ZbwrightDecohSym.tex}}\!} % Right decoherence	

	%% Y structure in B/W (light gray structure)
	\newcommand{\Ybwcolour}{black!20}
	\newcommand{\YbwdotSym}{\hbox{\input{symbols/YbwdotSym.tex}}\!\!} % Dot	
	\newcommand{\YbwcomultSym}{\hbox{\input{symbols/YbwcomultSym.tex}}\!\!} % Comultiplication	
	\newcommand{\YbwmultSym}{\hbox{\input{symbols/YbwmultSym.tex}}\!\!} % Multiplication	
	\newcommand{\YbwcounitSym}{\hbox{\input{symbols/YbwcounitSym.tex}}\!\!} % Counit
	\newcommand{\YbwunitSym}{\hbox{\input{symbols/YbwunitSym.tex}}\!\!} % Unit

	%% W structure in B/W (dark graystructure)
	\newcommand{\Wbwcolour}{black!50}
	\newcommand{\WbwdotSym}{\hbox{\input{symbols/WbwdotSym.tex}}\!\!} % Dot	
	\newcommand{\WbwcomultSym}{\hbox{\input{symbols/WbwcomultSym.tex}}\!\!} % Comultiplication	
	\newcommand{\WbwmultSym}{\hbox{\input{symbols/WbwmultSym.tex}}\!\!} % Multiplication	
	\newcommand{\WbwcounitSym}{\hbox{\input{symbols/WbwcounitSym.tex}}\!\!} % Counit
	\newcommand{\WbwunitSym}{\hbox{\input{symbols/WbwunitSym.tex}}\!\!} % Unit

	%% Traces	
	\newcommand{\traceSym}{\hbox{\input{symbols/traceSym.tex}}\!} % Trace symbol
	\newcommand{\smallTraceSym}{\hbox{\input{symbols/smallTraceSym.tex}}\!} % Small trace symbol for subscripts
	\newcommand{\cotraceSym}{\hbox{\input{symbols/cotraceSym.tex}}\!} % Co-trace symbol
	\newcommand{\trace}[1]{\traceSym_{#1}} % Trace
	\newcommand{\cotrace}[1]{\cotraceSym_{#1}} % Co-trace
	\newcommand{\traceSymAlt}{\top} % Alternative trace symbol
	\newcommand{\cotraceSymAlt}{\bot} % Alternative co-trace symbol
	\newcommand{\traceAlt}[1]{\traceSymAlt_{#1}} % Alternative trace
	\newcommand{\cotraceAlt}[1]{\cotraceSymAlt_{#1}} % Alternative co-trace

	%% Unlabelled symbols for controlled dynamics (algebras), projector-valued spectra (coalgebras), etx
	\newcommand{\algebraSym}{\hbox{\input{symbols/algebraSym.tex}}\!\!}	% Gray algebra symbol (2 inputs, 1 output)
	\newcommand{\measurementSym}{\hbox{\input{symbols/measurementSym.tex}}\!\!} % The adjoint of the algebra symbol
	\newcommand{\repSym}{\hbox{\input{symbols/repSym.tex}}\!\!} % Internalised representation G -> H x H*
	\newcommand{\mapSym}{\hbox{\input{symbols/mapSym.tex}}\!\!} % The same as the measurement symbol, but with white bg.
	\newcommand{\mapconjSym}{\hbox{\input{symbols/mapconjSym.tex}}\!\!} % The conjugate of the map symbol.

%% TIKZ

	\tikzset{
	  rectangle with rounded corners north west/.initial=4pt,
	  rectangle with rounded corners south west/.initial=4pt,
	  rectangle with rounded corners north east/.initial=4pt,
	  rectangle with rounded corners south east/.initial=4pt,
	}
	\makeatletter
	\pgfdeclareshape{rectangle with rounded corners}{
	  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
	  \inheritanchorborder[from=rectangle]
	  \inheritanchor[from=rectangle]{center}
	  \inheritanchor[from=rectangle]{north}
	  \inheritanchor[from=rectangle]{south}
	  \inheritanchor[from=rectangle]{west}
	  \inheritanchor[from=rectangle]{east}
	  \inheritanchor[from=rectangle]{north east}
	  \inheritanchor[from=rectangle]{south east}
	  \inheritanchor[from=rectangle]{north west}
	  \inheritanchor[from=rectangle]{south west}
	  \backgroundpath{% this is new
	    % store lower right in xa/ya and upper right in xb/yb
	    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
	    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
	    % construct main path
	    \pgfkeysgetvalue{/tikz/rectangle with rounded corners north west}{\pgf@rectc}
	    \pgfsetcornersarced{\pgfpoint{\pgf@rectc}{\pgf@rectc}}
	    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
	    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
	    \pgfkeysgetvalue{/tikz/rectangle with rounded corners north east}{\pgf@rectc}
	    \pgfsetcornersarced{\pgfpoint{\pgf@rectc}{\pgf@rectc}}
	    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
	    \pgfkeysgetvalue{/tikz/rectangle with rounded corners south east}{\pgf@rectc}
	    \pgfsetcornersarced{\pgfpoint{\pgf@rectc}{\pgf@rectc}}
	    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
	    \pgfkeysgetvalue{/tikz/rectangle with rounded corners south west}{\pgf@rectc}
	    \pgfsetcornersarced{\pgfpoint{\pgf@rectc}{\pgf@rectc}}
	    \pgfpathclose
	 }
	}
	\makeatother

	%% Arrowed arcs - WARNING: can cause "size" issues at compile time if arcs too small or crowded
	\tikzset{->-/.style={decoration={markings,mark=at position #1 with {\arrow{>}}},postaction={decorate}}}
	\tikzset{-<-/.style={decoration={markings,mark=at position #1 with {\arrow{<}}},postaction={decorate}}}

	\tikzstyle{every picture}=[baseline=-0.25em,scale=0.5]
	\pgfdeclarelayer{edgelayer}
	\pgfdeclarelayer{nodelayer}
	\pgfsetlayers{edgelayer,nodelayer,main}

	\tikzstyle{box} = [draw,shape=rectangle,inner sep=2pt,minimum height=6mm,minimum width=6mm,fill=white] 
	\tikzstyle{boxlarge} = [draw,shape=rectangle,inner sep=2pt,minimum height=1.5cm,minimum width=8mm,fill=white] 
	\tikzstyle{boxLarge} = [draw,shape=rectangle,inner sep=2pt,minimum height=2cm,minimum width=10mm,fill=white] 
	\tikzstyle{boxsmall} = [draw,shape=rectangle,inner sep=2pt,minimum height=3mm,minimum width=3mm,fill=white] % small in all directions. Might one day use boxnarrow for small in the largeness direction only.
	\tikzstyle{dot} = [inner sep=0mm,minimum width=3mm,minimum height=3mm,draw,shape=circle,text depth=-0.1mm]
	\tikzstyle{Zbwdot} = [dot, fill=\Zbwcolour]
	\tikzstyle{Xbwdot} = [dot, fill=\Xbwcolour]
	\tikzstyle{Ybwdot} = [dot, fill=\Ybwcolour]
	\tikzstyle{antipode} = [boxsmall] 

	%\tikzstyle{state} = [draw, rounded rectangle, rounded rectangle east arc=none,inner sep=2pt,minimum height=6mm,minimum width=6mm,fill=white]
	\tikzstyle{state} = [draw, rectangle with rounded corners,
	  rectangle with rounded corners north west=8pt,
	  rectangle with rounded corners south west=8pt,
	  rectangle with rounded corners north east=0pt,
	  rectangle with rounded corners south east=0pt,
	,inner sep=2pt,minimum height=6mm,minimum width=6mm,fill=white]
	\tikzstyle{statelarge} = [draw, rectangle with rounded corners,
	  rectangle with rounded corners north west=8pt,
	  rectangle with rounded corners south west=8pt,
	  rectangle with rounded corners north east=0pt,
	  rectangle with rounded corners south east=0pt,
	,inner sep=2pt,minimum height=1.5cm,minimum width=8mm,fill=white]
	\tikzstyle{stateLarge} = [draw, rectangle with rounded corners,
	  rectangle with rounded corners north west=8pt,
	  rectangle with rounded corners south west=8pt,
	  rectangle with rounded corners north east=0pt,
	  rectangle with rounded corners south east=0pt,
	,inner sep=2pt,minimum height=2cm,minimum width=8mm,fill=white]
	%\tikzstyle{effect} = [draw, rounded rectangle, rounded rectangle west arc=none,inner sep=2pt,minimum height=8mm,minimum width=6mm,fill=white]
	\tikzstyle{effect} = [draw, rectangle with rounded corners,
	  rectangle with rounded corners north west=0pt,
	  rectangle with rounded corners south west=0pt,
	  rectangle with rounded corners north east=8pt,
	  rectangle with rounded corners south east=8pt,
	,inner sep=2pt,minimum height=6mm,minimum width=6mm,fill=white]
	\tikzstyle{scalar}=[diamond,draw,inner sep=0.1mm,font=\small,fill=white]

	\tikzstyle{cdnode}=[fill=white]
	\tikzstyle{labelnode}=[fill=white]
	\tikzstyle{tightlabelnode}=[fill=white,inner sep = 0.1mm]
	\tikzstyle{none}=[inner sep=0pt]
	\tikzstyle{whiteline}=[-, line width=4pt, draw=white]

	\tikzstyle{trace}=[circuit ee IEC,thick,ground,scale=2.5]
	\tikzstyle{cotrace}=[circuit ee IEC,thick,ground,rotate=180,scale=2.5]
	\tikzstyle{upground}=[circuit ee IEC,thick,ground,rotate=90,scale=2.5]
	\tikzstyle{downground}=[circuit ee IEC,thick,ground,rotate=-90,scale=2.5]
	
	\tikzstyle{doubled} = [line width=1.8pt] % [line width=1.6pt] % [very thick]
	



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% End:


==> Generalised Mermin-type non-locality arguments/packages.tex <==
%%%% packages.tex by Stefano Gogioso 
%%%% Version 1 Aug 2016

%% MATHS %%
\usepackage{mathtools} % Loads and extends amsmath
\usepackage{amssymb} % Extram mathematical symbols (loads amsfonts)
\usepackage{bbold} % Sans-serif blackboard bold font for numbers
\usepackage{amsthm} % Theorem environments
%\usepackage{stmaryrd} % Some maths symbols for logic and computer science
%\usepackage{cjhebrew} % Jewish symbols
%\usepackage[nodisplayskipstretch]{setspace} % Redefines spacing before/after equations

%% WRITING %%
%\usepackage{relsize} % Additional relative sizes for fonts
\usepackage{microtype} % Improves appearance of writing
%\usepackage{fullpage} % Reduces lateral page margins for articles. Comment out for journal-specific document classes
%\usepackage{multicol} % Multi-column environments
\usepackage{csquotes} % Environments for quotes
%\usepackage{fancyvrb} % Verbatim environments
%\usepackage{ragged2e}
\usepackage{enumerate}

%% CITATIONS %%
\usepackage{hyperref} % Hyperlink citations. Comment out for arxiv submission
%\usepackage[nocompress]{cite} % Comment out if using natbib 
%\usepackage[round,authoryear,sort&compress]{natbib} % Comment out if using cite
%\usepackage{apacite}

%% GRAPHICS %%
\usepackage{graphicx} % To import graphics
%\usepackage{subcaption} % Captioning and referencing sub-figures
\usepackage[usenames,dvipsnames]{xcolor} % Introduces colour names
\usepackage{tikz} % TikZ
\usepackage{circuitikz} % TikZ circuit diagrams 
\usetikzlibrary{
	arrows,
	shapes,
	decorations,
	intersections,
	backgrounds,
	positioning,
	circuits.ee.IEC
	}

%% INPUT %%
%\usepackage[applemac]{inputenc} % Support for non-standard characters from macbook keyboard
%\usepackage[italian]{babel} % Support for italian accented characters




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% End:

